From Xception to NEXcepTion: New Design Decisions and Neural Architecture Search

In this paper, we present a modified Xception architecture, the NEXcepTion network. Our network has significantly better performance than the original Xception, achieving top-1 accuracy of 81.5% on the ImageNet validation dataset (an improvement of 2.5%) as well as a 28% higher throughput. Another variant of our model, NEXcepTion-TP, reaches 81.8% top-1 accuracy, similar to ConvNeXt (82.1%), while having a 27% higher throughput. Our model is the result of applying improved training procedures and new design decisions combined with an application of Neural Architecture Search (NAS) on a smaller dataset. These findings call for revisiting older architectures and reassessing their potential when combined with the latest enhancements.

==> a_detailed_architecture.tex <==
A detailed architecture of NEXcepTion-S is available in Table \ref{tab:nexception_s}, and for NEXcepTion-TP is available in Table \ref{tab:nexception_tp}
\input{tab4_nexception-s_detailed}

\input{tab5_nexception-tp_detailed}

\begin{figure}[h]
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/accs/acc.pdf}
    \caption{Accuracy}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/loss/loss.pdf}
    \caption{Loss}
  \end{minipage}
\end{figure}
